FLUID: A Unified Evaluation Framework for Flexible Sequential Data

Modern ML methods excel when training data is IID, large-scale, and well labeled. Learning in less ideal conditions remains an open challenge. The sub-fields of few-shot, continual, transfer, and representation learning have made substantial strides in learning under adverse conditions; each affording distinct advantages through methods and insights. These methods address different challenges such as data arriving sequentially or scarce training examples, however often the difficult conditions an ML system will face over its lifetime cannot be anticipated prior to deployment. Therefore, general ML systems which can handle the many challenges of learning in practical settings are needed. To foster research towards the goal of general ML methods, we introduce a new unified evaluation framework - FLUID (Flexible Sequential Data). FLUID integrates the objectives of few-shot, continual, transfer, and representation learning while enabling comparison and integration of techniques across these subfields. In FLUID, a learner faces a stream of data and must make sequential predictions while choosing how to update itself, adapt quickly to novel classes, and deal with changing data distributions; while accounting for the total amount of compute. We conduct experiments on a broad set of methods which shed new insight on the advantages and limitations of current solutions and indicate new research problems to solve. As a starting point towards more general methods, we present two new baselines which outperform other evaluated methods on FLUID. Project page: https://raivn.cs.washington.edu/projects/FLUID/.

==> 08_broader_impact.tex <==
\section*{Broader Impact}
\label{sec:broad}

The broader impact of \emph{any} technology out there is dependent on the way the community decides to use it and this is especially true in case of technologies powered by AI/ML.

\paragraph{Pros}
ML systems that work in the wild via sequential learning from unknown distributions can help build solutions that are more powerful and useful in the ways that weren't possible earlier. The potential of learning on the edge devices using the streaming data is better suited to alleviate privacy concerns. Lastly, the current ML models rely on periodic refreshing to serve the ever-changing preferences of the public leading to a large carbon footprint. \litw could potentially result in ML systems that update models incrementally depending on the streaming data, resulting in reduced energy footprint which is better for the environment.

\paragraph{Cons}
While creating powerful models that operate at scale could be beneficial, they could also be abused by people to adapt predatory algorithms faster to benefit off the end-users' private data. Additionally, with more freedom provided to the learner, the bias amplification might become another concern. 



==> 09_acknowledgements.tex <==
\section*{Acknowledgements}
This work is in part supported by NSF IIS 1652052, IIS 17303166, DARPA N66001-19-2-4031, 67102239 and gifts from Allen Institute for Artificial Intelligence. We thank Jae Sung Park and Mitchell Wortsman for insightful discussions and Daniel Gordon for the pretrained MoCo weights.  

==> TabsFigs/knn+hybrid.tex <==
\begin{figure}[h]
    \makebox[\columnwidth][c]{\includegraphics[width=1.22\columnwidth]{TabsFigs/images/backbones.pdf}}
    \caption{Plot (a) shows the difference between supervised and MoCo pretraining in the initial stages of the sequence. Plot (b) compares a variety of methods and Prototype Tuning outperforms at all stages of the sequence. Plot (c) shows that NCM generalizes better to novel classes as network capacity increases.}
    \label{fig:backbones}
\end{figure}

==> TabsFigs/macs+ood.tex <==
\begin{figure}[h]
    \centering
    \makebox[\columnwidth][c]{\includegraphics[width=1.22\columnwidth]{TabsFigs/images/MACs+OOD.pdf}}
    %\includegraphics[width=\columnwidth]{TabsFigs/images/MACs+OOD.pdf}
    \caption{(a) and (b) compare the accuracy and MACs for various update strategies when fine-tuning and standard training, respectively. Plot (c) compares the ROC curves for out-of-distribution methods.}
    \label{fig:MACs+OOD}
\end{figure}






==> TabsFigs/main_table.tex <==
\begin{table*}[ht!]
\centering
\caption{{Performance of the suite of methods (outlined in Section~\ref{sec:methods}) across accuracy and compute metrics on sequence 5. We present several variants of accuracy - Overall, Mean-per-class as well as accuracy bucketed into 4 categories: Novel-Head, Novel-Tail, Pretrain-Head and Pretrain-Tail (Pretrain refers to classes present in the ImageNet-1K dataset). Sup. refers to Supervised and MoCo refers to He et al.~\citep{he2019momentum}. The best technique on every metric is in \textbf{bold}. Some methods could leverage caching of representations for efficiency, so, both GMACs are reported. GMACs do not include pretraining compute costs. See Table~\ref{tab:mainresultsr50} in Appendix~\ref{sec:r50res} for results with ResNet50 backbone.}}
\vspace{1em}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lc|cc|cc|cc|c@{}}
\toprule
Method                       & \begin{tabular}[c]{@{}c@{}}Pretrain\\ Strategy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Novel - \\ Head (>50) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrain - \\ Head (>50) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Novel - \\ Tail (<50) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrain - \\ Tail (<50) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mean} \\ \textbf{Per-Class} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Overall}\\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}GMACs$\downarrow$ \\  ($\times10^6$)\end{tabular} \\\midrule
\multicolumn{9}{c}{Backbone - Conv-4}\\
\midrule
\rowcolor[HTML]{EFEFEF}(a) Prototypical Networks          & Meta                                                               & ~~11.63                                                                                & ~~22.03                                                                                   & ~~6.90                                                                             & ~~13.26                                                                                   & ~~11.13                                                               & ~~15.98                                                       & ~~\textbf{0.06}                                                                                 \\

(b) MAML                        & Meta                                                               & ~~2.86                                                                                & ~~2.02                                                                                   & ~~0.15                                                                             & ~~0.10                                                                                   & ~~1.10                                                               & ~~3.64                                                       & 2.20                                                                            \\
\midrule
\multicolumn{9}{c}{Backbone - ResNet18}\\
\midrule
\rowcolor[HTML]{EFEFEF}(c) Prototypical Networks          & Meta                                                            & ~~8.64                                                                                & 16.98                                                                                  & ~~6.79                                                                             & 12.74                                                                                  & ~~9.50                                                               & 11.14                                                      & ~~0.15                                                                                 \\
(d) ConstellationNet          & Sup+Meta.                                                            & 39.26                                                                                & 65.35                                                                                  & 26.28                                                                             & 52.91                                                                                  & 40.21                                                               & 46.13                                                      & ~~0.16                                                                                 \\

(e) \rowcolor[HTML]{EFEFEF} Meta-Baseline    & Sup.+Meta                                                        & 40.47                                                                               & 67.03                                                                                  & 27.53                                                                            & 53.87                                                                                  & 40.23                                                              & 47.62                                                      & 0.16 / 5.73                                                       \\

(f) ProtoMAML          & Sup.+Meta                                                            & 42.65                                                                                & 69.48                                                                                  & 28.91                                                                             & 54.16                                                                                 & 42.94                                                               & 49.25                                                      & 5.73                                                                                 \\

\rowcolor[HTML]{EFEFEF} (f) SimpleCNAPS          & Sup.+Meta                                                            & 41.59                                                                                & 68.79                                                                                  & 25.79                                                                             & 52.16                                                                                 & 41.82                                                               & 48.23                                                      & 0.16                                                                                 \\

(g) Weight Imprinting & Sup. & 40.32                                                                                          & 67.46                                                & 15.35                                                                                       & 34.18                                                & 32.69                                                                         & 48.51     &  0.16 / 5.73                \\

\rowcolor[HTML]{EFEFEF} (h) OLTR & Sup.  & 40.83 &	40.00 &	17.27 &	13.85 & 27.77 &	45.06& 0.16 / 6.39\\

(i) LwF             & Sup.                                                          & 30.07 & 67.50 & ~~7.23 & 56.96 & ~31.02 & 48.76 & 22.58 / 45.16\\
\rowcolor[HTML]{EFEFEF}(j) EWC & Sup. & 39.03 & 70.84 & 16.59 & 47.18 & 34.89 & 50.39 & 12.29\\
(k) DER & Sup. & 35.34 & 74.41 & 10.64 & 52.05 & 32.30 & 49.07 & 11.29\\
\rowcolor[HTML]{EFEFEF} (l) ER-AML & Sup. & 39.03 & 70.84 & 16.59 & 47.18 & 34.89 & 50.39 & 12.29\\
(m) Fine-tune                    & Sup.                                                          & 43.41                                                                               & \textbf{77.29}                                                                                  & 23.56                                                                            & \textbf{58.77}                                                                                  & 41.54                                                              & 53.80                                                      & 0.16 / 5.73                                                                            \\
\rowcolor[HTML]{EFEFEF} (n) Standard Training            & Sup.                                                          & 38.51                                                                               & 68.14                                                                                  & 16.90                                                                            & 43.25                                                                                  & 33.99                                                              & 49.46                                                      & 11.29                                                                                \\
(o) NCM                          & Sup.                                                          & 42.35                                                                               & 72.69                                                                                  & \textbf{31.72}                                                                            & 56.17                                                                                  & 43.44                                                              & 48.62                                                      & ~~\textbf{0.15}                                                                                 \\

(p) \textbf{\ET~(Ours)}             & Sup.                                                          & \textbf{48.85}                                                                               & 75.70                                                                                  & 27.93                                                                            & 45.73                                                                                  & \textbf{43.61}                                                              & \textbf{58.16}                                                      & 0.16 / 5.73                                                       \\\midrule
\rowcolor[HTML]{EFEFEF}  (q) Weight Imprinting & MoCo &16.77 &26.98 &~~6.19 &~~8.69 & 12.60 & 22.90 & 0.16 / 5.73\\
(r) OLTR & MoCo  & 34.60 &	33.74 &	13.38  &	9.38 &	22.68 &	39.92 & 0.16 / 6.39\\
\rowcolor[HTML]{EFEFEF} (s) Fine-tune                    & MoCo                                                         & 14.49                                                                                & 27.59                                                                                  & ~~0.10                                                                             & 4.96                                                                                  & 8.91                                                              & 26.86                                                      & 0.16 / 5.73                                                                            \\
(q) Standard Training            & MoCo                                                         & 26.63                                                                               & 45.02                                                                                  & ~~9.63                                                                             & 20.54                                                                                  & 21.12                                                              & 35.60                                                      & 11.29                                                                                \\
\rowcolor[HTML]{EFEFEF} (r) NCM                          & MoCo                                                         & 19.24                                                                               & 31.12                                                                                  & 14.40                                                                            & 21.95                                                                                  & 18.99                                                              & 22.90                                                      & ~~0.15                                                                                 \\
% (o) LwF & MoCo & & & & & & &22.58 \\

(s) \textbf{\ET~(Ours)}             & MoCo                                                         & 31.50                                                                               & 46.21                                                                                  & 12.90                                                                             & 21.10                                                                                  & 24.36                                                              & 39.61                                                      & 0.16 / 5.73                                                       \\\bottomrule
\end{tabular}}
\label{tab:mainresults}
\end{table*}

==> TabsFigs/metrics_old.tex <==
\begin{table*}[ht!]
\centering
\caption{\small{The evaluation metrics used in the \litw framework to capture the performance and capabilities of various algorithms.}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Metric}                         & \textbf{Description}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \toprule
Overall Accuracy           & The accuracy over all elements in the sequence.                                                                                                                                                                                                                                                                                                                                                                                                                                          \\\midrule
Mean Per Class Accuracy    & The accuracy for each class in the sequence averaged over all classes.                                                                                                                                                                                                                                                                                                                                                                      \\\midrule
Total Compute              & \begin{tabular}[c]{@{}l@{}}The total numbers of multiply-accumulate operations for all updates and evaluations accrued\\ over the sequence measured in GMACs (Giga MACs).\end{tabular}                                                                                                                                                                                                    \\\midrule
Unseen Class Detection     & \begin{tabular}[c]{@{}l@{}}The area under the receiver operating characteristic (AUROC) for the detection of samples\\ that are from previously unseen classes.\end{tabular}                                                                                                                                                                                           \\\midrule
Cross-Sectional Accuracies & \begin{tabular}[c]{@{}l@{}}The mean-class accuracy among classes in the sequence that belong to one of the 4 subcategories:\\ 1) \textit{Pretraining-Head}: Classes with $> 50$ samples that were included in pretraining.\\ 2) \textit{Pretraining-Tail}: Classes with $\leq 50$ samples that were included in pretraining.\\ 3) \textit{Novel-Head}: Classes with $> 50$ samples that were not included in pretraining.\\ 4) \textit{Novel-Tail}: Classes with $\leq 50$ samples that were not included in pretraining.\end{tabular} \\ \bottomrule
\end{tabular}
}
\label{tab:metrics} 
\end{table*}
